Developing a Resource-Constraint EdgeAI model for Surface Defect Detection

Resource constraints have restricted several EdgeAI applications to machine learning inference approaches, where models are trained on the cloud and deployed to the edge device. This poses challenges such as bandwidth, latency, and privacy associated with storing data off-site for model building. Training on the edge device can overcome these challenges by eliminating the need to transfer data to another device for storage and model development. On-device training also provides robustness to data variations as models can be retrained on newly acquired data to improve performance. We, therefore, propose a lightweight EdgeAI architecture modified from Xception, for on-device training in a resource-constraint edge environment. We evaluate our model on a PCB defect detection task and compare its performance against existing lightweight models - MobileNetV2, EfficientNetV2B0, and MobileViT-XXS. The results of our experiment show that our model has a remarkable performance with a test accuracy of 73.45% without pre-training. This is comparable to the test accuracy of non-pre-trained MobileViT-XXS (75.40%) and much better than other non-pre-trained models (MobileNetV2 - 50.05%, EfficientNetV2B0 - 54.30%). The test accuracy of our model without pre-training is comparable to pre-trained MobileNetV2 model - 75.45% and better than pre-trained EfficientNetV2B0 model - 58.10%. In terms of memory efficiency, our model performs better than EfficientNetV2B0 and MobileViT-XXS. We find that the resource efficiency of machine learning models does not solely depend on the number of parameters but also depends on architectural considerations. Our method can be applied to other resource-constraint applications while maintaining significant performance.

==> Contents/tables/edge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccllll@{}}
\toprule
\multicolumn{2}{c}{} &
  \multicolumn{1}{c}{Embedded Edge   Devices} &
  \multicolumn{1}{c}{Edge Nodes/   Edge Servers/ Edge Computers/ Micro Data} &
  \multicolumn{1}{c}{Edge Routers/   Edge Switches/ Edge Gateways} &
  \multicolumn{1}{c}{Edge Accelerator} \\ \midrule
\multicolumn{1}{|c|}{\multirow{2}{*}{Processing Power}} &
  \multicolumn{1}{c|}{CPU} &
  \multicolumn{1}{l|}{Low-power   processors} &
  \multicolumn{1}{l|}{General-purpose   processors} &
  \multicolumn{1}{l|}{Customized   processors} &
  \multicolumn{1}{l|}{Specialized   AI processors} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{GPU} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Optimized   GPU architecture} \\ \midrule
\multicolumn{2}{|c|}{Memory} &
  \multicolumn{1}{l|}{Limited   RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} \\ \midrule
\multicolumn{2}{|c|}{Storage} &
  \multicolumn{1}{l|}{Limited   flash storage} &
  \multicolumn{1}{l|}{Moderate   to high storage (HDD/SSD)} &
  \multicolumn{1}{l|}{Moderate   to high storage (HDD/SSD)} &
  \multicolumn{1}{l|}{Limited   storage (on-chip)} \\ \midrule
\multicolumn{2}{|c|}{Network} &
  \multicolumn{1}{l|}{Basic   connectivity} &
  \multicolumn{1}{l|}{Ethernet,   Wi-Fi, Cellular} &
  \multicolumn{1}{l|}{Ethernet,   Wi-Fi, Cellular} &
  \multicolumn{1}{l|}{Ethernet,   PCIe} \\ \midrule
\multicolumn{2}{|c|}{AI Support} &
  \multicolumn{1}{l|}{Limited   or no support} &
  \multicolumn{1}{l|}{Can   support AI frameworks and algorithms} &
  \multicolumn{1}{l|}{Limited   support for AI inference} &
  \multicolumn{1}{l|}{Optimized   for AI inference} \\ \midrule
\multicolumn{2}{|c|}{Power/Energy Consumption} &
  \multicolumn{1}{l|}{Low   power consumption} &
  \multicolumn{1}{l|}{Moderate   power consumption} &
  \multicolumn{1}{l|}{Moderate   power consumption} &
  \multicolumn{1}{l|}{Moderate   to high power consumption} \\ \midrule
\multicolumn{1}{|c|}{\multirow{3}{*}{Durability (Environment Resistant)}} &
  \multicolumn{1}{c|}{Shock   vs Vibration} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Temperature} &
  \multicolumn{1}{l|}{No} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{No} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Waterproof} &
  \multicolumn{1}{l|}{No} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{No} \\ \midrule
\multicolumn{2}{|c|}{Price} &
  \multicolumn{1}{l|}{Low} &
  \multicolumn{1}{l|}{Moderate   to high} &
  \multicolumn{1}{l|}{Moderate   to high} &
  \multicolumn{1}{l|}{High} \\ \midrule
\multicolumn{2}{|c|}{Typical Application} &
  \multicolumn{1}{l|}{Kiosk   machines, Building automation, Environmental monitoring, Industrial robotics} &
  \multicolumn{1}{l|}{Railway   signaling systems, Industrial data centers, Smart cities infrastructure} &
  \multicolumn{1}{l|}{Industrial   control systems, Industrial gateways, Smart manufacturing systems} &
  \multicolumn{1}{l|}{Video   surveillance and analytics, Autonomous vehicles and robotics} \\ \midrule
\multicolumn{2}{|c|}{Areas of Applications} &
  \multicolumn{1}{l|}{Sensor   devices, wearables, IoT devices} &
  \multicolumn{1}{l|}{Edge   computing, cloud offloading, data processing} &
  \multicolumn{1}{l|}{Network   routing, connectivity, data aggregation} &
  \multicolumn{1}{l|}{AI   inference, machine learning} \\ \midrule
\multicolumn{2}{|c|}{Example of Devices} &
  \multicolumn{1}{l|}{Arduino,   Raspberry Pi} &
  \multicolumn{1}{l|}{Industrial   edge servers, NVIDIA Jetson,Dell Edge Gateway} &
  \multicolumn{1}{l|}{Cisco   IoT routers, Juniper Networks} &
  \multicolumn{1}{l|}{NVIDIA   Tesla T4, Google TPU} \\ \midrule
\multicolumn{2}{|c|}{Drawbacks} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\ \midrule
\multicolumn{2}{c}{I/O} &
   &
   &
   &
   \\ \bottomrule
\end{tabular}%
}
% \end{table}

==> Contents/tables/edgeDevice.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{p{5em}p{5em}p{10em}p{12em}p{10em}p{10em}}
\hline
\hline
\multicolumn{2}{c}{} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Embedded} \\ \textbf{Edge Devices}\end{tabular}} &
%\multicolumn{1}{c|}{Embedded Edge Devices} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Nodes {\slash}} \\ \textbf{Edge Servers {\slash}} \\ \textbf{Edge Computers {\slash}} \\ \textbf{Micro Datacenter}\end{tabular}} &
%\multicolumn{1}{c|}{Edge Nodes {\slash} Edge Servers {\slash} Edge Computers {\slash} Micro Data Center} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Routers {\slash}} \\ \textbf{Edge Switches {\slash}} \\ \textbf{Edge Gateways}\end{tabular}} &
%\multicolumn{1}{c|}{Edge Routers {\slash} Edge Switches {\slash} Edge Gateways} &
\multicolumn{1}{c}{\textbf{Edge Accelerators}} \\ \hline
\multicolumn{2}{c}{Processing Power} &
Micro-controller, Low-power processors {\newline}\textit{e.g., AVR, PIC} &
  General purpose processors (up to 64 cores); GPU Supported 
  {\newline} \textit{e.g., Intel Atom, Intel Celeron, Xeon Processor}  &
  General purpose processors (4 to 56 cores); 
  {\newline} \textit{e.g., 2nd Generation Intel Xeon Scalable} &
  Specialized   AI processors; GPU Supported
  {\newline} \textit{e.g., Intel VPU, Google TPU, FPGA, Apple NPU}  \\ \hline
\multicolumn{2}{c}{Memory} &
  Up to 8MB; {\newline} \textit{e.g., SRAM} &
  Up to 256GB; {\newline} \textit{e.g., DDR4 RDIMM{\slash}LR-DIMM} &
  Up to 64GB; {\newline}\textit{e.g., DRAM} &
  Up to 8GB; {\newline} \textit{e.g., GDDR6, SDRAM, LPDDR4} \\ \hline
\multicolumn{2}{c}{Storage} &
  Up to 16MB {\newline} \textit{e.g., MicroSD}& 
  8GB to 6TB; {\newline} \textit{e.g., NVMe, SSD, MicroSD, eMMC} &
  Up to 2TB; {\newline} \textit{e.g., NVMe, SSD, SATA} &
  Up to 128GB; {\newline} \textit{e.g., eMMC, MicroSD}\\ \hline
\multicolumn{2}{c}{Network} &
  Bluetooth, Wi-Fi &
  Ethernet, Wi-Fi, Cellular &
  Ethernet, Wi-Fi, Cellular &
  Ethernet \\ \hline
\multicolumn{2}{c}{I/O} &
  Limited
  {\newline} \textit{e.g., USB, Ethernet} &
  Vary
  {\newline} \textit{PCIe, OCP, LOM, USB, iDRAC network port, Display ports} &
  Vary
  {\newline} \textit{Display ports, USB, uSIM slots, COM, Digital I/O} &
  Vary
  {\newline} \textit{PCIe, USB, HDMI, uSDHC, GPIO} \\ \hline
\multicolumn{2}{c}{AI Optimization} &
  Not Supported &
  Not Supported &
  Not Supported &
  Optimized for AI inference \\ \hline
\multicolumn{2}{c}{Power Consumption} &
  Low &
  Moderate &
  Moderate &
  Moderate to High \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{Durability}} &
  {\begin{tabular}[c]{@{}c@{}}{Shock \&} \\ {Vibration}\end{tabular}} &
  % Shock\&Vibration &
  Some Application Supports &
  Some Application Supports &
  Some Application Supports &
  Not Supported \\ \cline{2-6} 
\multicolumn{1}{c}{} &
  Temperature &
  -40C to 85C &
  -40C to 85C &
  -20C to 60C &
  -40C to 85C  \\ \cline{2-6} 
\multicolumn{1}{c}{} &
  Waterproof &
  Some Application Supports &
  Some Application Supports &
  Some Application Supports &
  No \\ \hline
\multicolumn{2}{c}{Price} &
  \$ &
  \$\$\$ &
  \$\$\$ &
  \$\$\$\$\$ \\ \hline
\multicolumn{2}{c}{Example of Devices} &
  Arduino &
  Raspberry Pi, Industrial Edge servers, NVIDIA Jetson&
  Cisco IoT routers, Juniper Networks, Dell Edge Gateway  &
  % NVIDIA Tesla T4, 
  Google Coral, Nvidia Jetson Nano, Intel Neural Compute Stick \\ \hline
\multicolumn{2}{c}{Typical Application} &
  Sensor devices, wearables, IoT devices, smart appliances\cite{9904804}\cite{8951147} &  
  Kiosk machines, Building automation, Environmental monitoring, Industrial robotics, Railway signaling systems, Industrial data centers, Smart cities infrastructure\cite{JIANG2020556} &
  Industrial control systems, Industrial gateways, Smart manufacturing systems &
  Video surveillance and analytics, Autonomous vehicles and robotics, Real time object detection \cite{park2020real}  \\ \hline

% \multicolumn{2}{|c|}{Reference} &
%   & 
%   &
%   &\\ \hline
\end{tabular}%
%}
% \end{table}






% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \begin{table}[]
% \centering
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{|p{5em}p{5em}|p{10em}|p{12em}|p{10em}|p{10em}|}
% \hline
% \hline
% \multicolumn{2}{|c|}{} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Embedded} \\ \textbf{Edge Devices}\end{tabular}} &
% %\multicolumn{1}{c|}{Embedded Edge Devices} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Nodes {\slash}} \\ \textbf{Edge Servers {\slash}} \\ \textbf{Edge Computers {\slash}} \\ \textbf{Micro Datacenter}\end{tabular}} &
% %\multicolumn{1}{c|}{Edge Nodes {\slash} Edge Servers {\slash} Edge Computers {\slash} Micro Data Center} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Routers {\slash}} \\ \textbf{Edge Switches {\slash}} \\ \textbf{Edge Gateways}\end{tabular}} &
% %\multicolumn{1}{c|}{Edge Routers {\slash} Edge Switches {\slash} Edge Gateways} &
% \multicolumn{1}{c|}{\textbf{Edge Accelerators}} \\ \hline
% \multicolumn{2}{|c|}{Processing Power} &
%   Micro-processor, Micro-controller; (Low-power   processors) &
%   Quad-Core, Hvbrid-Core (General purpose processors); Intel Atom, Intel Celeron, Xeon Processor; GPU Supported &
%   4 to 56 core processors (Customizable); 2nd Generation Intel Xeon Scalable processors &
%   CPU, GPU, VPU, TPU, FPGA, NPU (Specialized   AI processors) \\ \hline
% \multicolumn{2}{|c|}{Memory} &
%   Up to 8MB; {\newline} SRAM &
%   Up to 256GB; {\newline} DDR4 RDIMM{\slash}LR-DIMM &
%   Up to 64GB;  &
%   Up to 4GB; {\newline} GDDR6, SDRAM, LPDDR4 \\ \hline
% \multicolumn{2}{|c|}{Storage} &
%   Up to 16MB &
%   8GB to 6TB; {\newline} NVMe, SSD, MicroSD, eMMC &
%   Up to 2TB; {\newline} NVMe, SSD, SATA &
%   Up to 16GB; {\newline} eMMC, MicroSD\\ \hline
% \multicolumn{2}{|c|}{Network} &
%   Bluetooth, Wi-Fi &
%   Ethernet, Wi-Fi, Cellular &
%   Ethernet, Wi-Fi, Cellular &
%   Ethernet \\ \hline
% \multicolumn{2}{|c|}{AI Optimization} &
%   Not Supported &
%   Not Supported &
%   Not Supported &
%   Optimized for AI inference \\ \hline
% \multicolumn{2}{|c|}{Power Consumption} &
%   Low power consumption &
%   Moderate power consumption &
%   Moderate power consumption &
%   Moderate to high power consumption \\ \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Durability}} &
%   {\begin{tabular}[c]{@{}c@{}}{Shock \&} \\ {Vibration}\end{tabular}} &
%   % Shock\&Vibration &
%   Some Application Supports &
%   Some Application Supports &
%   Some Application Supports &
%   Not Supported \\ \cline{2-6} 
% \multicolumn{1}{|c|}{} &
%   Temperature &
%   -40C to 85C &
%   -40C to 85C &
%   -20C to 60C &
%   -40C to 85C  \\ \cline{2-6} 
% \multicolumn{1}{|c|}{} &
%   Waterproof &
%   Some Application Supports &
%   Some Application Supports &
%   Some Application Supports &
%   No \\ \hline
% \multicolumn{2}{|c|}{Price} &
%   \$ &
%   \$\$ to \$\$\$ &
%   \$\$ to \$\$\$ &
%   \$\$\$ \\ \hline
% \multicolumn{2}{|c|}{Typical Application} &
%   Sensor devices, wearables, IoT devices, smart appliances\cite{9904804}\cite{8951147} &  
%   Kiosk machines, Building automation, Environmental monitoring, Industrial robotics, Railway signaling systems, Industrial data centers, Smart cities infrastructure\cite{JIANG2020556} &
%   Industrial control systems, Industrial gateways, Smart manufacturing systems &
%   Video surveillance and analytics, Autonomous vehicles and robotics \\ \hline
% \multicolumn{2}{|c|}{Example of Devices} &
%   Arduino &
%   Raspberry Pi, Industrial edge servers, NVIDIA Jetson,Dell Edge Gateway &
%   Cisco IoT routers, Juniper Networks &
%   % NVIDIA Tesla T4, 
%   Google Coral TPU \\ \hline
% \multicolumn{2}{|c|}{I/O} &
%   USB, Ethernet &
%   PCIe, OCP, LOM, USB, iDRAC network port, Display ports &
%   Display ports, USB, uSIM slots, COM, Digital I/O &
%   PCIe, USB, HDMI, uSDHC, GPIO \\ \hline
% % \multicolumn{2}{|c|}{Reference} &
% %   & 
% %   &
% %   &\\ \hline
% \end{tabular}%
% %}
% % \end{table}

==> Contents/tables/testing_results.tex <==
\begin{tabular}{llllll}
\hline\hline
\textbf{Model} & \textbf{Parameters}  & \textbf{Test Acc} & \textbf{Inference Time} & \textbf{Mem Usage} & \textbf{Power Cons} \\
\hline
Xception-Lite & 11.2M & \textbf{73.45\%} & 35s & 1493.1 MB & XXXX \\
MobileNetV2 & 2.2M & 50.05\% & \textbf{22s} & 1745.2 MB & XXXX \\
EfficientNetV2B0 & 5.9M & 54.30\% & 28s & 1451.8 MB & XXXX \\
MobileViT-XXS & \textbf{1.3M} & 50.00\% & 48s & \textbf{1135.7 MB} & XXXX \\
% Xception & 20M & XXXX & 1120s & XXXXX \\
\hline
\end{tabular}

